Margin-based sampling in high dimensions: When being active is less efficient than staying passive

It is widely believed that given the same labeling budget, active learning (AL) algorithms like margin-based active learning achieve better predictive performance than passive learning (PL), albeit at a higher computational cost. Recent empirical evidence suggests that this added cost might be in vain, as margin-based AL can sometimes perform even worse than PL. While existing works offer different explanations in the low-dimensional regime, this paper shows that the underlying mechanism is entirely different in high dimensions: we prove for logistic regression that PL outperforms margin-based AL even for noiseless data and when using the Bayes optimal decision boundary for sampling. Insights from our proof indicate that this high-dimensional phenomenon is exacerbated when the separation between the classes is small. We corroborate this intuition with experiments on 20 high-dimensional datasets spanning a diverse range of applications, from finance and histology to chemistry and computer vision.

==> app_proofcorrolaries.tex <==
\subsection{Proof of Corollary~\ref{cor:oracleuncertainty}}
\label{sec:cororacleproof}

In Theorem~\ref{thm:oracleuncertainty}, let
us denote the numerators of the expressions of $\alphaor$ and $\alphaPL$ by
$\marginminor$ and $\marginminPL$, respectively. Similarly, we
use the notation $\Mor, \MPL$ for the denominators of $\alphaor$
and $\alphaPL$, respectively.

Since the function $\Psifull$ defined in Equation~\ref{eq:testerror} is monotonic in
$\alpha$, it follows from Theorem~\ref{thm:oracleuncertainty} with high
probability that oracle margin-based sampling performs worse than passive
learning if $\alphaor = \frac{\marginminor}{\Mor} > \frac{\marginminPL}{\MPL} =
\alphaPL$. We observe that
% Using the notation $\Mor$ and $\marginminor$\footnote{Note that while
% $\marginminor$ and $\marginminAL$ refer to the margin defined in
% Equation~\ref{eq:margin}, $\marginminPL$ corresponds to the \emph{average}
% margin defined in Equation~\ref{eq:avgmargin}.} $$. We observe that

\begin{equation*}
\frac{\marginminor}{\Mor}> \frac{\marginminPL}{\MPL} \iff \frac{\marginminor}{\marginminPL} > \frac{\Mor}{\MPL}
\end{equation*}

For an $\eta \in (0, 1)$ and using the expressions for $\marginminor$ and
$\marginminPL$ from Theorem~\ref{thm:oracleuncertainty}, we have that

\begin{equation*}
\frac{\marginminor}{\marginminPL} > \eta \iff d > \nlab \frac{\left(1+t+\eta\sqrt{2
t \nlab^{-1/2}}\right)^2}{(1-\eta)^2}
\end{equation*}

Moreover, for $\eta > \frac{\Mor}{\MPL}$, we find that
\begin{equation*}
\eta > \frac{\Mor}{\MPL} \iff \mean_{tr} > \frac{\passiveratio(\mean_{tr}+t
  \stdsig_{tr}\nseed^{-1/2}) +  6.059(1-\passiveratio)\cdot 10^{-2} \mean_{tr} +
t \stdsig_{tr} \nlab^{-1/2} \eta }{\eta}
\end{equation*}

Hence, by plugging in $\eta = 0.5$, we have that $\frac{\marginminor}{\Mor}> \frac{\marginminPL}{\MPL}$ if 
\begin{align}
  \frac{d}{\nlab} &> 4 \left(1+t+\sqrt{t (4\nlab)^{-1/2}}\right)^2 \label{eq:cond_d}\\
  \mean_{tr} &> 2 \passiveratio(\mean_{tr}+t\stdsig_{tr}\nseed^{-1/2}) +
  2\cdot 6.059(1-\passiveratio)\cdot 10^{-2} \mean_{tr} + 2t \stdsig_{tr} \nlab^{-1/2}
\end{align}

% We find the condition on $\mean_{tr}$ by using the condition that 
Using $\passiveratio < 0.5$ we arrive at 
\begin{equation*}
\mean_{tr}> \frac{ t \stdsig_{tr} (1 + 2\passiveratio^{1/2})\nlab^{-1/2}}{1 -2\passiveratio}
\end{equation*}

We now solve for $\passiveratio$ and find

\begin{equation*}
\sqrt{\passiveratio} < q\left(\sqrt{1+\frac{1}{2 q^2}-\frac{1}{q}}-1\right)
\end{equation*}

\noindent with $q = \frac{t \stdsig_{tr}}{2 \mean_{tr} \sqrt{\nlab}}$.
Using the fact that $\sqrt{\passiveratio} < \frac{1}{\sqrt{2}}$ and ignoring
negligible terms, we get the following bound on $\passiveratio$
% For clarity, we also approximate by using that $\passiveratio^{1/2} < \frac{1}{\sqrt{2}}$ and find the looser bound

\begin{equation*}
\passiveratio < \frac{1}{2}-\frac{1+\sqrt{2}}{2} \frac{t \stdsig_{tr}}{\sqrt{\nlab} \mean_{tr}}
\end{equation*}
which concludes the proof.
%\begin{equation} \mean_{tr} > 2 \frac{ \nquery 6.059 \cdot 10^{-2} \nquery
%\mean_{tr}+ t \stdsig_{tr} (\sqrt{\nlab} -%\sqrt{\nseed})}{\nlab-2\nseed}
%\end{equation}

\subsection{Proof of Corollary~\ref{cor:cortwostageproof}}
\label{sec:cortwostageproof}

Similar to Section~\ref{sec:cororacleproof}, let us denote in
Theorem~\ref{thm:uncertaintysampling} the numerators of the expressions of
$\alphaUS$ and $\alphaPL$ by $\marginminAL$ and $\marginminPL$, respectively.
Similarly, we use the notation $\MUS, \MPL$ for the denominators of $\alphaUS$
and $\alphaPL$, respectively.

By Theorem~\ref{thm:uncertaintysampling} margin-based sampling leads to a
classifier with a lower test error than uniform sampling, if $\alphaUS =
\frac{\marginminAL}{\MUS} \geq \frac{\marginminPL}{\MPL} = \alphaPL$. Similar to
the proof of Corollary~\ref{cor:oracleuncertainty}, we find that

\begin{equation*}
\frac{\marginminAL}{\MUS} \geq \frac{\marginminPL}{\MPL} \iff \frac{\marginminAL}{\marginminPL} \geq \frac{\MUS}{\MPL} 
\end{equation*}
Let $\eta \in (0, 1)$. Then it holds that
\begin{equation*}
\begin{aligned}
\frac{\marginminAL}{\marginminPL} \geq \eta &\iff \sqrt{d/\nlab}-\sqrt{2
\log \nunl} -1 -t \geq \eta \left( \sqrt{d/\nlab+2 t\nlab^{-1/2}} \right)\\
&\Rightarrow \sqrt{d/\nlab}-\sqrt{2 \log \nunl} -1 -t \geq \eta \left(
\sqrt{d/\nlab}+\sqrt{2 t\nlab^{-1/2}} \right)\\
&\iff d/\nlab > \frac{\sqrt{2 \log \nunl} + 1+ t +\eta\sqrt{2 t\nlab^{-1/2}}}{(1-\eta)^2}
\end{aligned}
\end{equation*}
Choosing $\eta = 0.5$ yields
\begin{equation*}
  d/\nlab > 4\left(\sqrt{2 \log \nunl} + 1+ t +\sqrt{ t (4\nlab)^{-1/2}}\right)
\end{equation*}

Similarly, we have that $\frac{\MUS}{\MPL}< \eta$. Plugging in the expressions given in Theorem~\ref{thm:uncertaintysampling}, we find that

\begin{equation*}
\label{eq:cseed}
\passiveratio \Cseed + (1-\passiveratio) \left(6.059 \cdot 10^{-2}\mean_{tr} + \left(
    \frac{2 \log \nunl}{\Cseed}\right)^{1/2}\left(\frac{d}{\passiveratio \nlab}+\frac{2 \stdsig_{tr}t}{\passiveratio \nlab}\right)^{1/4}+t
\right)< \eta \left( \mean_{tr} - \frac{t\stdsig_{tr}}{\nlab^{1/2}} \right)
\end{equation*}

% First, we note that if the seed set classifier is trivial, i.e.
% $\alpha_{seed}$ is very large, than two stage uncertainty sampling queries
% points without any information on the signal. Observe that the larger
% $\mean_{tr}$ the larger the signal component in the seed set, namely $\Cseed$.
Recalling the bound on $\Cseed$ in Equation~\ref{eq:upperboundcseed}, we find that if

\begin{equation}
\label{eq:meanbound1}
\mean_{tr}  \geq \left(\frac{d}{\passiveratio  \nlab}+ \frac{2 \stdsig_{tr} t}{\rho \nlab} \right)^{1/6}(2 \log \nunl)^{1/3} + \frac{t\stdsig_{tr}}{(\passiveratio  \nlab)^{1/2}} 
\end{equation}


\noindent then the following condition on $\passiveratio$ suffices in order to
guarantee that $\alphaPL < \alphaUS$:

\begin{equation*}
  \passiveratio <   \frac{0.878 \mean_{tr}-t \stdsig_{tr}(\passiveratio
\nlab)^{-1/2} - \left(\frac{d}{\passiveratio  \nlab}+ \frac{\stdsig_{tr} t}{
\passiveratio  \nlab} \right)^{1/6}(2 \log \nunl)^{1/3} -t}{\Cseed}
\end{equation*}


==> related_work.tex <==
\section{Related work}
\label{sec:related_work}

% In this section, we discuss related work regarding the prior analysis of
% uncertainty sampling, active learning in high-dimensions and batch active
% learning.

%\fy{in the context of mitigation somewhere? - cite label complexity exponential gain stuff for sparse half-spaces low -noise
%  though now there's even some for noise ~1/2 - see slack. some theoreticians might be reminded immediately}

\fy{i think this one can be fused with the corresponding paragraph in intro}
\paragraph{Prior analyses of uncertainty sampling.} As mentioned in
Section~\ref{sec:intro}, prior experimental works on a broad variety
of datasets and applications both confirm \citep{tong01, settles07,
  schohn20, raj21} and contradict the intuition \citep{schein07,
  lughofer17, yang18, siddhant18} that uncertainty sampling leads to significant gains
compared to uniform sampling.
%% show that in line with intuition,
%% uncertainty sampling leads to significant gains on a broad variety of datasets and applications
%% \citep{tong01, settles07, schohn20, raj21}. In contrast, a number of works \citep{schein07, lughofer17,                     
%% yang18, siddhant18} show experimentally that uncertainty sampling sometimes     
%% leads to worse performance than uniform sampling (i.e.\ passive learning).
\fy{Several works tried to characterize failure cases of uncertainty sampling, 
  in the low-dimensional regime:}
\citet{mussmann18} prove that the benefits of uncertainty sampling are          
proportional to the Bayes error for a given low-dimensional data distribution. 
Furthermore, \citet{huang14} shows that uncertainty sampling may acquire skewed
data. While these works shed light on uncertainty sampling in
low dimensions, to the best of our knowledge, little is known about uncertainty
sampling in the high-dimensional regime.
\fy{following sentence seems to fit better here as well?}
There are a plethora of works considering active learning in the large sample
size regime \citep{Balcan07, balcan13, Zhang21, Gentile22, chen17, yan17,
haupt11}. In contrast, we show that in the low sample size regime a different
intuition is necessary.

%Complementing these experimental
%observations, 
% a number of recent theoretical works analyze uncertainty sampling. For
% instance,
%\citet{raj21} show that considering a linear classifier, uncertainty sampling
%converges to a solution with good generalization. Moreover, \citet{brinker03} showed that by adding a diversity metric uncertainty sampling can easily successfully be used in batch-active learning. 

%\fy{hae where are the standard exponential sample complexity gain papers here?
%even if low-dim, why is halfspace stuff not here?} the reason is that they are
%not exactly uncertainty sampling.

%Despite these positive results, 
%In contrast, a number of works \citep{schein07, lughofer17,
%yang18, siddhant18} show experimentally that uncertainty sampling sometimes
%leads to worse performance than uniform sampling (i.e.\ passive learning).  In addition,
%\citet{mussmann18} prove that the benefits of uncertainty sampling are
%proportional to the Bayes error for a given low-dimensional data distribution.
%Furthermore, \citet{huang14} shows that uncertainty sampling may acquire skewed
%data.
\fy{merge into intro}
\paragraph{Active learning in high dimensions.} In the context of learning
half-spaces \fy{for $s$-sparse ground truths?}
%under sparsity assumptions,
the work of \citet{Zhang18} provides sample
complexity results in high dimensions by using a method close to uncertainty
sampling adjusted with basis pursuit \fy{penalized by $\ell_1$ norm} and analyzing existing large-sample
size query methods \citep{haupt11, dasgupta05, awasthi14, chen17, yan17} with
basis pursuit. \fy{the bounds are the same as for uniform sampling, one-bit CS?}

We conjecture that for $n < \log d$ and uniform sampling with
basis pursuit the phenomenon discussed in Section \ref{sec:theory} persists.
\fy{On a completely different line of work blabla}
  experiments in \citep{ducoffe18, sener18, shui20, mahmood21} suggest that                      
margin-based sampling strategies for neural networks are rarely better          
than uniform sampling for image data. We make the same observation on common
computer vision datasets in Section
\ref{sec:exp_verify_theory} and show evidence that the phenomenon discussed in
Section \ref{sec:theory} can be the cause. 


%where this effect is amplified by batch active learning, which is often
%employed in deep learning applications \citep{sener18, Kirsch2019, gissin19,
%shui20}. Techniques such as  distribution matching
%  \citep{yang15, gal17, gissin19} or importance sampling \citep{farquhar2021}
%  attempt to mitigate these issues for settings with large labeling budgets.
%discuss the problems that arise due to the fact
%that the data acquired via uncertainty sampling is skewed and not representative
%of the training distribution.  This effect is further amplified by batch active
%learning, which is often employed in deep learning applications \citep{sener18,
%  Kirsch2019, gissin19, shui20}. Techniques like distribution matching
%  \citep{yang15, gal17, gissin19} or importance sampling \citep{farquhar2021}
%  attempt to mitigate these issues for settings with large query budgets.
%While these works paint a detailed picture of uncertainty sampling in
%Despite the detailed picture in low dimensions, little is known about how effective this sampling
%strategy is for high-dimensional data and small labeling budgets. However, experiments in
%\citep{ducoffe18, sener18, shui20, mahmood21} suggest that
%margin-based sampling strategies for neural networks are rarely better
%than uniform sampling for image data. Even though these experiments indicate a serious shortcoming of uncertainty sampling in high dimensions,
%to the best of our knowledge, no prior work has tried to investigate
%this phenomenon further (either theoretically or empirically).

\fy{merge with 4.6}
\paragraph{Other active learning algorithms.} 
Lastly, we note that in deep learning, it is common to
use batch-active learning \citep{brinker03, sener18, Kirsch2019, gissin19, shui20}.
\fy{hence bla argue that for DL experiments, U-AL might be bad because of batch effects}
However, \citet{huang14} argues that batch-active learning amplifies the effect
\fy{of bad uncertainty score?}
of acquiring skewed data.
To mitigate this issue of batch active learning,
\fy{Because of bad uncertainty score in particular in batch-active learning \citep{brinker03, sener18, Kirsch2019, gissin19, shui20}, people developed } techniques such as  distribution matching                              
\citep{yang15, gal17, gissin19} or importance sampling \citep{farquhar2021}.
 attempt to mitigate these issues \fy{repeat} for settings with large labeling budgets. In
 Section \ref{sec:experiments}, we show experimentally why these approaches may
 suffer from the same phenomenon by analyzing two distribution matching
 approaches: core-set and $\epsilon$-greedy sampling.

%Many works have focused on learning
%(sparse) half-spaces in the pool-based active learning framework and reported up
%to exponential gains in sample complexity by active learning compared to passive
%learning. However, many of these works focus on the low-dimensional regime $d<
%\nlab$ \citep{Balcan07, balcan13, Zhang21, Gentile22, chen17, yan17,
%haupt11}. In contrast, we show that
%a different intuition is necessary in the high-dimensional regime where $d \gg
%\nlab$. Moreover, we conjecture that assuming a sparse ground truth with similar
%methods to uncertainty sampling
%\citep{zhang18, haupt11, dasgupta05, awasthi14, chen17, yan17}
%we conjecture that, despite helping to achieve other
%desiderata like computational efficiency \citep{Zhang18},
%assuming a sparse
%ground truth 
%\fy{where does this suddenly come from?} \at{the only way to talk
%about this 58 in a meaningful way} 
%does not solve the failure cause discussed in Section \ref{sec:theory}: for
%$\nlab < \log d$ labeling samples in the neighborhood of the Bayes optimal
%decision boundary would still lead to poor generalization compared to uniform
%sampling. 
% Assuming a sparse ground truth can allow for computationally efficient active
% learning algorithms in low dimensions \citep{Zhang18}. On the other hand, in
% high dimensions assuming sparsity and using 
%Others study variants of uncertainty sampling with sparse ground truths
%\citep{Zhang18}, where in the very low sample size regime, we hypothesize that
%the methods have the same failure mode as uncertainty sampling. \fy{this sounds
%like laundry list sentene - they also show some expo gain?}\at{which one?} 
% Lastly, there is a large body of works that consider stream-based active
% learning for learning half-spaces \citep{Amin20, Hopkins20}, a significantly
% different problem from the pool-based setting we assume in this paper.

% \paragraph{Related problems.} Many of the core principles of active learning,
% such as the exploration-exploitation trade-off, also apply to other problems
% like Bayesian optimization \citep{frazier18}, offline reinforcement learning
% \citep{xie21, Jin2021} or bandit problems\at{cite}. We leave it as future work
% to study how our findings extend to these problems. \fy{this sounds like a
% future work paragraph? unless they did some analysis thats relevant to our
% phenomenon?}

% \paragraph{Other active learning strategies.} In addition, several works
% propose to query points using a score that combines uncertainty and a measure
% of how representative of the training distribution the samples are. These
% strategies too suffer from the problems we expose in Section~\ref{sec:theory},
% as long as they sample points close to the true decision boundary.

% \paragraph{Relationship to semi-supervised learning.} Both active learning and
% semi-supervised learning (SSL) are suitable in similar settings, namely when
% both a small labeled set and a large unlabeled set are available. Therefore, it
% is natural to wonder whether SSL could in fact entirely solve the problems shown
% by active learning in high dimensions. The issue with SSL, however, is that it
% requires strong assumptions to work well, while active learning can decrease the
% labeled sample complexity exponentially compared to passive (supervised)
% learning for a very broad family of distributions \citep{dasgupta05,
% beygelzimer10, Hanneke13}. For instance, \citet{causal12} argues that SSL cannot
% improve over supervised learning in causal learning problems (i.e.\ covariates
% $x$ are a causal parent of the predictor $y$), while active learning can still
% provide benefits in such scenarios. In particular, we highlight that the
% shortcomings of uncertainty sampling that we reveal in this paper also apply for
% causal learning problems, where SSL cannot be used either. 
% % \at{this paragraph needs to be 1/3 of what it is 

